Household Leverage Cycle Around the Great Recession

This paper provides the first causal evidence that credit supply expansion caused the 1999-2010 U.S. business cycle mainly through the channel of household leverage (debt-to-income ratio). Specifically, induced by net export growth, credit expansion in private-label mortgages, rather than government-sponsored enterprise mortgages, causes a much stronger boom and bust cycle in household leverage in the high net-export-growth areas. In addition, such a stronger household leverage cycle creates a stronger boom and bust cycle in the local economy, including housing prices, residential construction investment, and house-related employment. Thus, our results are consistent with the credit-driven household demand channel (Mian and Sufi, 2018). Further, we show multiple pieces of evidence against the corporate channel, which is emphasized by other business cycle theories (hypotheses).

==> App_DataDetails.tex <==
%------------------------------------------------------------
%------------------------------------------------------------


%------------------------------------------------------------
\subsection{Appendix for Data Details}\label{subsec:App_Data}


%------------------------------------------------------------
%------------------------------------------------------------
\subsubsection{HMDA Mortgage Data Processing Procedures at ZIP level}
In this section, I illustrate the processing details regarding the mortgage data at the ZIP code level. I will describe the processes of crosswalking from census tracts to ZIP codes, retaining data in the 1990-2000-unchanged ZIP codes, linking ZIP codes to primary counties and metropolitan areas, mortgage data requirement at the ZIP level, and grouping ZIP codes into income groups within metropolitan areas. 

\paragraph{Crosswalk from Census Tracts to ZIP Codes} 
First, I use the 712 or 800 consistent counties across time to filter HMDA data, depending on the period of interest. Second, HMDA mortgage data uses various versions of census tracts across time. 1981-1991, 1992-2002, and 2003-2009 HMDA datasets use 1980, 1990, and 2000 versions of the census tract, respectively. From the Missouri Census Data Center \footnote{Missouri Census Data Center's website is here: \url{https://mcdc.missouri.edu/applications/geocorr.html}}, I obtain the crosswalk file that links 1980 census tracts to 1990 ZIP codes, that links 1990 census tracts to 1990 ZIP codes, and that links 2000 census tracts to 2000 ZIP codes. I use population weight in the crosswalk since multiple census tracts can match multiple ZIP codes. I use 1992-1999 as the prior period for comparison because I intend to retain a reasonably large number of ZIP codes in a balanced panel for comparison. To prevent within-ZIP code changes from contaminating my analysis, I only keep ZIP codes that are mostly covered by HMDA reporting. Specifically, I keep ZIP codes with populations crosswalked from the HMDA mortgage data that are equal to or above 90\% of the ZIP total population. The deleted ZIP codes are mostly the ZIP codes on the boundary of metropolitan areas, since HMDA mainly covers metropolitan areas. 

ZIP codes are reasonably large areas within metropolitan areas. One ZIP code typically contains several census blocks, which are designed to provide more statistical uniformity with an average of 4,000 plus population. In the 1992-2009 mortgage panel data of 9995 ZIP codes, ZIP codes contain a population size of 4237, 12610, and 26023 at 25\%, 50\%, and 75\%, respectively. \footnote{For more information comparing census tracts and ZIP codes, see \url{https://proximityone.com/tracts_zips.htm}.}



\paragraph{Retaining Data in the 1990-2000-unchanged ZIP codes}
According to \cite{bailey2023national}, ZIP code geographic boundary can change in relationship to population growth and decline across time. For example, their detailed work based on The Postal Bulletin by the U.S. Postal Office shows that 3015 changes happened between 1990 and 2000. This number of changes is not small given 29,401 distinct ZIP codes were in operation at the beginning of 1990 (by the crosswalk file from the Missouri Census Data Center described above). Typical changes include merge, split, and boundary alteration. These changes can result in measurement error (matching observations to the wrong unites) or missing data (due to an observation reporting a ZIP code that did not in operation at the beginning of the sample period). 

To avoid the potential measurement error and missing data, I get a list of 1990-2000-unchanged ZIP codes by following steps. First, from the Missouri Census Data Center, I get the crosswalk file from 1990 ZIP codes to 1990 counties with population weights. Second, I delete any ZIP codes that may experience change during 1990-2000 from the 1990 ZIP codes list. Specifically, I delete ZIP codes that appear in the following variables in the following files by \cite{bailey2023national}: (1) variable ``oldzipcode" or ``newzipcode" in file ``ZIP\_Code\_Changes\_1990-2000\_Documentation.xls" and (2) ``zipcode" in file ``ZIP\_xwalk\_90-00.dta". Out of the 29,401 ZIP codes in the year 1990, 26,577 ZIP codes did not experience any change. Third, I match these ZIP codes to ZIP codes in the crosswalk file from 2000 ZIP codes to 2000 counties with population weights. I retain only matched ZIP codes. The above three steps result in 
26,058 1990-2000-unchanged ZIP codes. 

\paragraph{Link ZIP codes to Their Primary Counties and Metropolitan Areas}
One ZIP code can be linked to multiple counties (metropolitan areas) when it exists on the border. For each match zip code, I only keep its primary matched county that contains the most population in the zip code. From the Missouri Census Data Center, I get the crosswalk file that links 2000 ZIP codes to 2000 counties. I retain counties in the 2003 version of metropolitan areas in U.S. mainland (excluding Hawaii and Alaska).\footnote{Metropolitan areas definition (CBSA code) of 2003 can be found here: \url{https://www2.census.gov/programs\%2Dsurveys/metro\%2Dmicro/geographies/reference\%2Dfiles/2003/historical\%2Ddelineation\%2Dfiles/030606omb\%2Dnecta\%2Dcnecta.xls}.} 


The above steps result in 13,513 1990-2000-unchanged ZIP codes that are matched to primary counties in the metropolitan areas (2003 version CBSA code) in the U.S. mainland. I use these ZIP codes to filter HMDA ZIP-level data. 

 
\paragraph{Mortgage Data Requirement at the ZIP Level}\label{subsec:MortgageData_ZIP}
I require each ZIP code to have mortgage data in all years of analysis (1992-2009 for figure and 1999-2009 for regression analysis). I also require each ZIP code must have nonzero value for government-sponsored enterprise mortgages, private-label mortgages (non-jumbo), and mortgages retained on the balance sheet of financial institutions in the initial year (either 1992 or 1999). This requirement make sure that each ZIP code has starting value and non-missing growth rate in the main analysis.\footnote{This step also excludes ZIP codes with a tiny population.} The resulting 1992-2009 (1999-2009) mortgage panel data contains 9,995 (10,785) ZIP codes from 693 (782) counties.


\paragraph{Group ZIP codes Within Metropolitan Areas}
To conduct analysis in Section (\ref{subsec:ModelNewPrediction_Empirical})) for the model-based new predictions, I need to sum mortgage data in ZIP codes into half-, tertile-, quartile-, and quintile-income groups within metropolitan areas. To make sure each metropolitan statistic area (MSA) contains enough ZIP codes for calculation, I require that each MSA contains at least three ZIP codes for the calculation of half- and tertile-income groups and at least five ZIP codes for the calculation of quartile- and quintile-income groups. Since ZIP codes are reasonably large areas (with a population size of 4237 and 26023 at 25\% and 75\% in the 1992-2009 mortgage panel data), I believe three (five) ZIP codes are a good minimum number for the calculation.  



%------------------------------------------------------------
%------------------------------------------------------------
\subsubsection{House Price Data at ZIP level}
The annual house price index at the ZIP level based on repeat sales comes from the Federal Housing Financing Agency.\footnote{The data website of the Federal Housing Financing Agency is here: \url{https://www.fhfa.gov/DataTools/Downloads/Pages/House-Price-Index-Datasets.aspx#qexe}.} This database has reasonably good coverage of the ZIP codes of US metropolitan areas in and after 1992 (11,556 ZIP codes in 1992) but a little bit less coverage than the HMDA mortgage data.

\paragraph{Merge House Price and Mortgage Data at ZIP Level}
For both figure and regression analysis regarding house prices, I require that the ZIP codes are covered by both house price data and mortgage data refined in Section \ref{subsec:MortgageData_ZIP}. The merged data set contains fewer ZIP codes compared to mortgage data since house price data covers fewer ZIP codes. Second, I require that each zip code contains both data 1992-2009 (1999-2009) for figure (regression analysis). 


\paragraph{Interpolating House Units}
I collect the number of house units at the ZIP level from Decennial Census Summary Files in 1900 (File 3B), 2000 (File 1), and 2010 (File 1). Since Census data are collected as of March in 1990, 2000, and 2010, I treat the number of house units as the one at the end of last year (1989, 1999, and 2009, respectively). I interpolate the number of house units from 1990 to 2008 by a linear function. Then, I merge house unit data with the prices-mortgage merged data. For the final data, I require that each MSA contains at least three ZIP codes for the calculation of half- and tertile-income groups and at least five ZIP codes for the calculation of quartile- and quintile-income groups. 

Due to data availability of house prices and house units, the final data contains fewer ZIP codes than the mortgage data. The 1992-2009 half- (quintile-) income group data for figure contains 6,083 (5,942) ZIP codes from 244 (204) metropolitan areas. The 1999-2009 half- (quintile-) income group data for regression analysis contains 8,517 (8,427) ZIP codes from 293 (268) metropolitan areas.


\comment{
Lastly, I use the number of house units as weights to aggregate house prices across zip code groups within metropolitan areas. 
}

%################################################################################
%################################################################################
% This is the end of the entire section (tex file)
%################################################################################
%################################################################################

==> App_EmpCreditExpansion.tex <==
%------------------------------------------------------------
%------------------------------------------------------------
\subsection{Appendix for the Empirical: Supporting Credit Expansion}\label{subsec:App_EmpCreditExpansion}



%################################################################################
%################################################################################
% This is the end of the entire section (tex file)
%################################################################################
%################################################################################

==> Empirical.ConsumptionCycle.tex <==
%------------------------------------------------------------
%------------------------------------------------------------
\section{Empirical: Consumption Cycle (To be Done)}\label{subsec:Empirical.Consumption}
%------------------------------------------------------------
%------------------------------------------------------------
In this section, we show empirical evidence that credit-driven household leverage cycle results in a stronger boom and bust cycle in consumption in the high net-export-growth metropolitan areas. 











%################################################################################
%################################################################################
% This is the end of the entire section (tex file)
%################################################################################
%################################################################################

==> Empirical.DoubleDifference.tex <==
%------------------------------------------------------------
%------------------------------------------------------------
%\clearpage
%------------------------------------------------------------
%------------------------------------------------------------
\section{Empirical Results: ``Double Difference"}




















%################################################################################
%################################################################################
% This is the end of the entire section (tex file)
%################################################################################
%################################################################################

==> Table_HH/Old/table_Tradable.D00t06vsD07t10.NEP.D99t05.2SLS.ControlSet5.tex <==
%-----------------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table:Tradable.D00t06vsD07t10.PLMNJ.2SLS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Stacked Regression of Tradable Employment Growth in Boom (00-06) and Bust (07-10) Periods on Net Export Growth (99-05)} \smallskip \newline
{\scriptsize
This table reports 2SLS regression $\triangle_{00,06} \& \triangle_{07,10} TradableEmpShr_{c} = \beta_{00,06} * \triangle_{99,05} \text{NetExp}_{m} \times Dum_{00,06} + \beta_{07,10} * \triangle_{99,05} \text{NetExp}_{m} \times Dum_{07,10} + \gamma_{00,06}* \bm{Controls_{c}} \times Dum_{00,06} + \gamma_{07,10}* \bm{Controls_{c}} \times Dum_{07,10} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{00,06} \& \triangle_{07,10} TradableEmpShr_{c}$ is the change of the Tradable employment share in working-age population at county $c$ 00-06 and 07-10. The key independent variable $\triangle_{99,05} \text{NetExp}_{m}$ is the growth rate of net export growth at county $c$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in the period start year 1999. We use the gravity model-based instrumental variable $\triangle_{99,05}\text{givNetExp}_{m}$ as the IV for $\triangle_{99,05}\text{NetExp}_{m}$. Regression is weighted by the natural logarithm of housing units in 1999.  For the first-stage F-test of two non-stacked samples, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
\smallskip
} % end of small font size
} % end of caption
\label{table:Tradable.D00t06vsD07t10.PLMNJ.2SLS}

\vspace{-2mm}

\resizebox{0.55\columnwidth}{!}{%
\begin{tabular}{l*{5}{c}}
\toprule
\textbf{TSLS estimates}            &\multicolumn{5}{c}{Tradable Employment Growth (00-06 and 07-10, An)} \\
            \cmidrule{2-6} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
            
\midrule
Net Export Growth (99-05, An) x Dum00t06&    0.790***&    0.804***&    0.701***&    0.742***&    0.690***\\
               &  (0.191)   &  (0.191)   &  (0.173)   &  (0.174)   &  (0.177)   \\
\addlinespace
Net Export Growth (99-05, An) x Dum07t10&    0.783***&    0.814***&    0.776***&    0.835***&    0.742***\\
               &  (0.215)   &  (0.228)   &  (0.249)   &  (0.259)   &  (0.255)   \\
\addlinespace
Dum00t06       &   -0.001***&    0.004   &    0.007   &    0.045***&    0.048***\\
               &  (0.000)   &  (0.006)   &  (0.007)   &  (0.016)   &  (0.015)   \\
\addlinespace
Dum07t10       &   -0.002***&    0.009   &    0.004   &    0.057***&    0.068***\\
               &  (0.000)   &  (0.007)   &  (0.009)   &  (0.019)   &  (0.022)   \\
\addlinespace
Ln(Num of HH, 99) x DumD00t06&            &   -0.000   &    0.006*  &    0.007*  &    0.005   \\
               &            &  (0.000)   &  (0.004)   &  (0.004)   &  (0.004)   \\
\addlinespace
Ln(Num of HH, 99) x DumD07t10&            &   -0.000   &    0.000   &    0.000   &    0.000   \\
               &            &  (0.000)   &  (0.002)   &  (0.002)   &  (0.002)   \\
\addlinespace
Ln(HH Income, 99) x DumD00t06&            &   -0.000   &   -0.001   &   -0.004***&   -0.004***\\
               &            &  (0.001)   &  (0.001)   &  (0.002)   &  (0.001)   \\
\addlinespace
Ln(HH Income, 99) x DumD07t10&            &   -0.000   &   -0.000   &   -0.005***&   -0.006***\\
               &            &  (0.001)   &  (0.001)   &  (0.002)   &  (0.002)   \\
\addlinespace
Ratio of Labor Force (1999) x DumD00t06&            &    0.000   &   -0.004   &   -0.005   &   -0.005   \\
               &            &  (0.004)   &  (0.004)   &  (0.004)   &  (0.005)   \\
\addlinespace
Ratio of Labor Force (1999) x DumD07t10&            &   -0.009** &   -0.006   &   -0.006   &   -0.009*  \\
               &            &  (0.004)   &  (0.004)   &  (0.005)   &  (0.005)   \\
\addlinespace
Ln(Num of HU, 99) x DumD00t06&            &            &   -0.006*  &   -0.007*  &   -0.006   \\
               &            &            &  (0.004)   &  (0.004)   &  (0.004)   \\
\addlinespace
Ln(Num of HU, 99) x DumD07t10&            &            &   -0.000   &   -0.001   &   -0.001   \\
               &            &            &  (0.002)   &  (0.002)   &  (0.002)   \\
\addlinespace
Housing supply elasticity x DumD00t06&            &            &    0.000   &    0.000   &    0.000   \\
               &            &            &  (0.000)   &  (0.000)   &  (0.000)   \\
\addlinespace
Housing supply elasticity x DumD07t10&            &            &   -0.000   &   -0.000   &   -0.000   \\
               &            &            &  (0.000)   &  (0.000)   &  (0.000)   \\
\addlinespace
House Vacancy Rate (1999) x DumD00t06&            &            &    0.012** &    0.011** &    0.009   \\
               &            &            &  (0.006)   &  (0.006)   &  (0.006)   \\
\addlinespace
House Vacancy Rate (1999) x DumD07t10&            &            &    0.009** &    0.007*  &    0.009** \\
               &            &            &  (0.004)   &  (0.004)   &  (0.004)   \\
\addlinespace
Ratio of Renters (1999) x DumD00t06&            &            &   -0.002   &   -0.006** &   -0.007** \\
               &            &            &  (0.002)   &  (0.003)   &  (0.003)   \\
\addlinespace
Ratio of Renters (1999) x DumD07t10&            &            &    0.001   &   -0.006** &   -0.009***\\
               &            &            &  (0.002)   &  (0.003)   &  (0.003)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x DumD00t06&            &            &            &    0.011** &    0.007   \\
               &            &            &            &  (0.005)   &  (0.005)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x DumD07t10&            &            &            &    0.014***&    0.003   \\
               &            &            &            &  (0.005)   &  (0.005)   \\
\addlinespace
Ratio of White Race (1999) x DumD00t06&            &            &            &    0.001   &    0.000   \\
               &            &            &            &  (0.001)   &  (0.001)   \\
\addlinespace
Ratio of White Race (1999) x DumD07t10&            &            &            &   -0.001   &   -0.002   \\
               &            &            &            &  (0.002)   &  (0.002)   \\
\addlinespace
Ratio of Immigration (90-00) x DumD00t06&            &            &            &    0.012   &    0.017*  \\
               &            &            &            &  (0.008)   &  (0.009)   \\
\addlinespace
Ratio of Immigration (90-00) x DumD07t10&            &            &            &    0.022** &    0.025***\\
               &            &            &            &  (0.009)   &  (0.009)   \\
\addlinespace
Ratio of Art, Enter, and Recre Emp (1999) x DumD00t06&            &            &            &            &    0.052***\\
               &            &            &            &            &  (0.020)   \\
\addlinespace
Ratio of Art, Enter, and Recre Emp (1999) x DumD07t10&            &            &            &            &    0.042** \\
               &            &            &            &            &  (0.021)   \\
\addlinespace
Ratio of Health Emp (1999) x DumD00t06&            &            &            &            &    0.053***\\
               &            &            &            &            &  (0.016)   \\
\addlinespace
Ratio of Health Emp (1999) x DumD07t10&            &            &            &            &    0.047** \\
               &            &            &            &            &  (0.019)   \\
\addlinespace
Ratio of Tradable Service Emp (1999) x DumD00t06&            &            &            &            &    0.012   \\
               &            &            &            &            &  (0.012)   \\
\addlinespace
Ratio of Tradable Service Emp (1999) x DumD07t10&            &            &            &            &    0.047***\\
               &            &            &            &            &  (0.018)   \\
\addlinespace
Ratio of College Students (1999) x DumD00t06&            &            &            &            &   -0.022** \\
               &            &            &            &            &  (0.010)   \\
\addlinespace
Ratio of College Students (1999) x DumD07t10&            &            &            &            &    0.004   \\
               &            &            &            &            &  (0.010)   \\
\midrule
Obs            &     1578   &     1578   &     1396   &     1396   &     1396   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   \\
KP F-Stat (99-05, non-stack sample)       &    23.44   &    23.20   &    16.52   &    17.83   &    17.17   \\
MOP F-Stat (99-05, non-stack sample)  &    22.98   &    22.71   &    16.16   &    17.49   &    16.88   \\
CoefEqual\_Chi2  &    0.001   &    0.002   &    0.117   &    0.183   &    0.054   \\
CoefEqual\_PValue  &    0.973   &    0.961   &    0.732   &    0.669   &    0.816   \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}

==> Table_HH/Old/table_Tradable.D00t06vsD07t10.NEP.D99t05.2SLS.wide.ControlSet5.tex <==
%-----------------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_Tradable.D00t06vsD07t10.NEP.D99t05.2SLS.wide
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Stacked Regression of Tradable Employment Growth in Boom (00-06) and Bust (07-10) Periods on Net Export Growth (99-05)} \smallskip \newline
{\scriptsize
This table reports 2SLS regression $\triangle_{00,06} \& \triangle_{07,10} TradableEmpShr_{c} = \beta_{00,06} * \triangle_{99,05} \text{NetExp}_{m} \times Dum_{00,06} + \beta_{07,10} * \triangle_{99,05} \text{NetExp}_{m} \times Dum_{07,10} + \gamma_{00,06}* \bm{Controls_{c}} \times Dum_{00,06} + \gamma_{07,10}* \bm{Controls_{c}} \times Dum_{07,10} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{00,06} \& \triangle_{07,10} TradableEmpShr_{c}$ is the change of the Tradable employment share in working-age population at county $c$ 00-06 and 07-10. The key independent variable $\triangle_{99,05} \text{NetExp}_{m}$ is the growth rate of net export growth at county $c$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in the period start year 1999. We use the gravity model-based instrumental variable $\triangle_{99,05}\text{givNetExp}_{m}$ as the IV for $\triangle_{99,05}\text{NetExp}_{m}$. Regression is weighted by the natural logarithm of housing units in 1999.  For the first-stage F-test of two non-stacked samples, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
\smallskip
} % end of small font size
} % end of caption
\label{table_Tradable.D00t06vsD07t10.NEP.D99t05.2SLS.wide}

\vspace{-2mm}

\resizebox{\columnwidth}{!}{%
\begin{tabular}{l*{10}{c}}
\toprule
\textbf{TSLS estimates}            &\multicolumn{10}{c}{Tradable Employment Growth (00-06 and 07-10, An)} \\
            \cmidrule{2-11} 
            &\multicolumn{2}{c}{(1)}&\multicolumn{2}{c}{(2)}&\multicolumn{2}{c}{(3)}&\multicolumn{2}{c}{(4)}&\multicolumn{2}{c}{(5)} \\
            
\midrule
Net Export Growth (99-05, An) x Dum00t06&    0.790***&  (0.191)&    0.804***&  (0.191)&    0.701***&  (0.173)&    0.742***&  (0.174)&    0.690***&  (0.177)\\ 
\addlinespace
Net Export Growth (99-05, An) x Dum07t10&    0.783***&  (0.215)&    0.814***&  (0.228)&    0.776***&  (0.249)&    0.835***&  (0.259)&    0.742***&  (0.255)\\  \addlinespace
Dum00t06       &   -0.001***&  (0.000)&    0.004   &  (0.006)&    0.007   &  (0.007)&    0.045***&  (0.016)&    0.048***&  (0.015)\\  \addlinespace
Dum07t10       &   -0.002***&  (0.000)&    0.009   &  (0.007)&    0.004   &  (0.009)&    0.057***&  (0.019)&    0.068***&  (0.022)\\  \addlinespace
Ln(Num of HH, 99) x DumD00t06&            &         &   -0.000   &  (0.000)&    0.006*  &  (0.004)&    0.007*  &  (0.004)&    0.005   &  (0.004)\\  \addlinespace
Ln(Num of HH, 99) x DumD07t10&            &         &   -0.000   &  (0.000)&    0.000   &  (0.002)&    0.000   &  (0.002)&    0.000   &  (0.002)\\  \addlinespace
Ln(HH Income, 99) x DumD00t06&            &         &   -0.000   &  (0.001)&   -0.001   &  (0.001)&   -0.004***&  (0.002)&   -0.004***&  (0.001)\\  \addlinespace
Ln(HH Income, 99) x DumD07t10&            &         &   -0.000   &  (0.001)&   -0.000   &  (0.001)&   -0.005***&  (0.002)&   -0.006***&  (0.002)\\  \addlinespace
Ratio of Labor Force (1999) x DumD00t06&            &         &    0.000   &  (0.004)&   -0.004   &  (0.004)&   -0.005   &  (0.004)&   -0.005   &  (0.005)\\  \addlinespace
Ratio of Labor Force (1999) x DumD07t10&            &         &   -0.009** &  (0.004)&   -0.006   &  (0.004)&   -0.006   &  (0.005)&   -0.009*  &  (0.005)\\  \addlinespace
Ln(Num of HU, 99) x DumD00t06&            &         &            &         &   -0.006*  &  (0.004)&   -0.007*  &  (0.004)&   -0.006   &  (0.004)\\  \addlinespace
Ln(Num of HU, 99) x DumD07t10&            &         &            &         &   -0.000   &  (0.002)&   -0.001   &  (0.002)&   -0.001   &  (0.002)\\  \addlinespace
Housing supply elasticity x DumD00t06&            &         &            &         &    0.000   &  (0.000)&    0.000   &  (0.000)&    0.000   &  (0.000)\\  \addlinespace
Housing supply elasticity x DumD07t10&            &         &            &         &   -0.000   &  (0.000)&   -0.000   &  (0.000)&   -0.000   &  (0.000)\\  \addlinespace
House Vacancy Rate (1999) x DumD00t06&            &         &            &         &    0.012** &  (0.006)&    0.011** &  (0.006)&    0.009   &  (0.006)\\  \addlinespace
House Vacancy Rate (1999) x DumD07t10&            &         &            &         &    0.009** &  (0.004)&    0.007*  &  (0.004)&    0.009** &  (0.004)\\  \addlinespace
Ratio of Renters (1999) x DumD00t06&            &         &            &         &   -0.002   &  (0.002)&   -0.006** &  (0.003)&   -0.007** &  (0.003)\\  \addlinespace
Ratio of Renters (1999) x DumD07t10&            &         &            &         &    0.001   &  (0.002)&   -0.006** &  (0.003)&   -0.009***&  (0.003)\\  \addlinespace
Ratio of Bachelor Educated (1999) x DumD00t06&            &         &            &         &            &         &    0.011** &  (0.005)&    0.007   &  (0.005)\\  \addlinespace
Ratio of Bachelor Educated (1999) x DumD07t10&            &         &            &         &            &         &    0.014***&  (0.005)&    0.003   &  (0.005)\\  \addlinespace
Ratio of White Race (1999) x DumD00t06&            &         &            &         &            &         &    0.001   &  (0.001)&    0.000   &  (0.001)\\  \addlinespace
Ratio of White Race (1999) x DumD07t10&            &         &            &         &            &         &   -0.001   &  (0.002)&   -0.002   &  (0.002)\\  \addlinespace
Ratio of Immigration (90-00) x DumD00t06&            &         &            &         &            &         &    0.012   &  (0.008)&    0.017*  &  (0.009)\\  \addlinespace
Ratio of Immigration (90-00) x DumD07t10&            &         &            &         &            &         &    0.022** &  (0.009)&    0.025***&  (0.009)\\  \addlinespace
Ratio of Art, Enter, and Recre Emp (1999) x DumD00t06&            &         &            &         &            &         &            &         &    0.052***&  (0.020)\\  \addlinespace
Ratio of Art, Enter, and Recre Emp (1999) x DumD07t10&            &         &            &         &            &         &            &         &    0.042** &  (0.021)\\  \addlinespace
Ratio of Health Emp (1999) x DumD00t06&            &         &            &         &            &         &            &         &    0.053***&  (0.016)\\  \addlinespace
Ratio of Health Emp (1999) x DumD07t10&            &         &            &         &            &         &            &         &    0.047** &  (0.019)\\  \addlinespace
Ratio of Tradable Service Emp (1999) x DumD00t06&            &         &            &         &            &         &            &         &    0.012   &  (0.012)\\  \addlinespace
Ratio of Tradable Service Emp (1999) x DumD07t10&            &         &            &         &            &         &            &         &    0.047***&  (0.018)\\  \addlinespace
Ratio of College Students (1999) x DumD00t06&            &         &            &         &            &         &            &         &   -0.022** &  (0.010)\\  \addlinespace
Ratio of College Students (1999) x DumD07t10&            &         &            &         &            &         &            &         &    0.004   &  (0.010)\\  \addlinespace
\midrule
Obs             &     1578   &         &     1578   &         &     1396   &         &     1396   &         &     1396   &         \\
Cluster SE      &     CBSA   &         &     CBSA   &         &     CBSA   &         &     CBSA   &         &     CBSA   &         \\
Weight         & Ln(HU99)   &         & Ln(HU99)   &         & Ln(HU99)   &         & Ln(HU99)   &         & Ln(HU99)   &         \\
KP F-Stat (99-05, non-stack sample)      &    23.44   &         &    23.20   &         &    16.52   &         &    17.83   &         &    17.17   &         \\
MOP F-Stat (99-05, non-stack sample)  &    22.98   &         &    22.71   &         &    16.16   &         &    17.49   &         &    16.88   &         \\
CoefEqual\_Chi2  &    0.001   &         &    0.002   &         &    0.117   &         &    0.183   &         &    0.054   &         \\
CoefEqual\_PValue &    0.973   &         &    0.961   &         &    0.732   &         &    0.669   &         &    0.816   &         \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}

==> Table_HH/Old/table_Tradable.D00t06vsD07t10.NEP.D99t05.4Reg.ControlSet5.tex <==
%---------------------------------------------------------------

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_Tradable.D00t06vsD07t10.NEP.D99t05.4Reg
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{Four Stacked Regressions of Tradable Employment Growth in Boom (00-06) and Bust (07-10) Periods on Net Export Growth (99-05)} \smallskip \newline
{\scriptsize
This table reports OLS, reduced-form, first stage, and second stages of stacked 2SLS regression $\triangle_{00,06} \& \triangle_{07,10} TradableEmpShr_{c} = \beta_{00,06} * \triangle_{99,05} \text{NetExp}_{m} \times Dum_{00,06} + \beta_{07,10} * \triangle_{99,05} \text{NetExp}_{m} \times Dum_{07,10} + \gamma_{00,06}* \bm{Controls_{c}} \times Dum_{00,06} + \gamma_{07,10}* \bm{Controls_{c}} \times Dum_{07,10} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{00,06} \& \triangle_{07,10} TradableEmpShr_{c}$ is the change of the Tradable employment share in working-age population at county $c$ 00-06 and 07-10. The key independent variable $\triangle_{99,05} \text{NetExp}_{m}$ is the growth rate of net export growth at county $c$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in the period start year 1999. We use the gravity model-based instrumental variable $\triangle_{99,05}\text{givNetExp}_{m}$ as the IV for $\triangle_{99,05}\text{NetExp}_{m}$. Regression is weighted by the natural logarithm of housing units in 1999.  For the first-stage F-test of two non-stacked samples, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
} % end of small font size
} % end of caption
\label{table_Tradable.D00t06vsD07t10.NEP.D99t05.4Reg}
\resizebox{0.95\columnwidth}{!}{%
\begin{tabular}{l*{5}{c}}
\toprule
Dep Var (Panel A, B, and C)                      &\multicolumn{5}{c}{Tradable Employment Growth (00-06 \& 07-10, An)} \\
            \cmidrule{2-6} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\multicolumn{1}{c}{(5)} \\     


\midrule
\multicolumn{6}{l}{\textbf{Panel A. OLS estimates}} \\
Net Export Growth (99-05, An) x Dum00t06&    0.537***&    0.544***&    0.472***&    0.451***&    0.406***\\
               &  (0.104)   &  (0.103)   &  (0.099)   &  (0.097)   &  (0.101)   \\
\addlinespace
Net Export Growth (99-05, An) x Dum07t10&    0.625***&    0.638***&    0.599***&    0.576***&    0.495***\\
               &  (0.149)   &  (0.155)   &  (0.163)   &  (0.154)   &  (0.153)   \\
\addlinespace
R2-adj         &    0.427   &    0.430   &    0.449   &    0.459   &    0.475   \\
\addlinespace


\midrule
\multicolumn{6}{l}{\textbf{Panel B. Reduced-form estimates}} \\
GIV Net Export Growth (99-05, An) x Dum00t06&    0.910***&    0.921***&    0.772***&    0.831***&    0.738***\\
               &  (0.187)   &  (0.183)   &  (0.180)   &  (0.168)   &  (0.179)   \\
\addlinespace
GIV Net Export Growth (99-05, An) x Dum07t10&    0.903***&    0.932***&    0.854***&    0.936***&    0.794***\\
               &  (0.176)   &  (0.179)   &  (0.188)   &  (0.190)   &  (0.197)   \\
\addlinespace
R2-adj         &    0.413   &    0.416   &    0.437   &    0.454   &    0.471   \\
\addlinespace


\midrule
\multicolumn{6}{l}{\textbf{Panel C . 2SLS estimates}} \\
\addlinespace
Net Export Growth (99-05, An) x Dum00t06&    0.790***&    0.804***&    0.701***&    0.742***&    0.690***\\
               &  (0.191)   &  (0.191)   &  (0.173)   &  (0.174)   &  (0.177)   \\
\addlinespace
Net Export Growth (99-05, An) x Dum07t10&    0.783***&    0.814***&    0.776***&    0.835***&    0.742***\\
               &  (0.215)   &  (0.228)   &  (0.249)   &  (0.259)   &  (0.255)   \\
               
\addlinespace
\addlinespace

Dep Var (Panel D): &\multicolumn{5}{c}{Net Export Growth (99-05, An)} \\ 
\midrule 
\multicolumn{6}{l}{\textbf{Panel D . First-stage estimates only for 99-05 (Non-stack sample)}} \\
\addlinespace
GIV NEG (99-05, An)&    1.153***&    1.145***&    1.101***&    1.121***&    1.069***\\
               &  (0.238)   &  (0.238)   &  (0.271)   &  (0.265)   &  (0.258)   \\
\addlinespace
KP F-Stat      &    23.44   &    23.20   &    16.52   &    17.83   &    17.17   \\
MOP F-Stat     &    22.98   &    22.71   &    16.16   &    17.49   &    16.88   \\
\addlinespace



\midrule
\multicolumn{6}{l}{\textbf{Controls (for all Panels)}} \\
DumPeriod  &    Y        &  Y   &   Y    & Y    &  Y    \\
Basic Controls x DumPeriod &            &  Y   &   Y    & Y    &  Y    \\
Housing Controls x DumPeriod &           &      & Y       & Y    &  Y    \\
Demographic Controls x DumPeriod &            &      &        &  Y    &  Y    \\
Industry Controls x DumPeriod &            &      &        &      &  Y    \\

\midrule              
Obs (Panel A, B, and C)          &     1578   &     1578   &     1396   &     1396   &     1396   \\
Obs (Panel D)          &      789   &      789   &      698   &      698   &      698   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   \\
\bottomrule
\end{tabular}

} % end of resize box

\end{table}


==> Table_HH/table_BEAConstEmp.D00t06vsD07t10.HHDTI.2SLS.tex <==
%-----------------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_BEAConstEmp.D00t06vsD07t10.HHDTI.2SLS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Stacked Regression of BEA Construction Employment Growth in Boom (00-06) and Bust (07-10) Periods on Household Leverage Rise (99-05)} \smallskip \newline
{\scriptsize
This table reports 2SLS regression $\triangle_{00,06} \& \triangle_{07,10} BEAConstEmpShr_{c} = \beta_{00,06} * \triangle_{99,05} HHDTI_{c} \times Dum_{00,06} + \beta_{07,10} * \triangle_{99,05} HHDTI_{c} \times Dum_{07,10} + \gamma_{00,06}* \bm{Controls_{c}} \times Dum_{00,06} + \gamma_{07,10}* \bm{Controls_{c}} \times Dum_{07,10} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{00,06} \& \triangle_{07,10} BEAConstEmpShr_{c}$ is the change of the BEA construction employment share in working-age population at county $c$ 00-06 and 07-10. To reduce the impact of outliers, the dependent variable is winsorized at 2\% and 98\% levels in each period. The key independent variable $\triangle_{99,05} HHDTI_{c}$ is the rise in household leverage (debt-to-income ratio) at county $c$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in the period start year 1999. We use the gravity model-based instrumental variable $\triangle_{99,05}\text{givNetExp}_{m}$ as the IV for $\triangle_{99,05}HHDTI_{c}$. Regression is weighted by the natural logarithm of housing units in 1999. For the first-stage F-test of two non-stacked samples, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
\smallskip
} % end of small font size
} % end of caption
\label{table_BEAConstEmp.D00t06vsD07t10.HHDTI.2SLS}

\vspace{-2mm}

\resizebox{0.55\columnwidth}{!}{%
\begin{tabular}{l*{4}{c}}
\toprule
\textbf{TSLS estimates}            &\multicolumn{4}{c}{BEA Construction Employment Growth (00-06 and 07-10, An)} \\
            \cmidrule{2-5} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
            
\midrule
HH Debt-to-Income Rise (99-05, An) x Dum00t06&    0.022** &    0.020** &    0.018   &    0.019** \\
               &  (0.011)   &  (0.009)   &  (0.011)   &  (0.010)   \\
\addlinespace
HH Debt-to-Income Rise (99-05, An) x Dum07t10&   -0.030***&   -0.023** &   -0.024*  &   -0.025** \\
               &  (0.012)   &  (0.010)   &  (0.014)   &  (0.011)   \\
\addlinespace
Dum00t06       &   -0.002   &    0.009   &   -0.005   &    0.012   \\
               &  (0.002)   &  (0.010)   &  (0.006)   &  (0.013)   \\
\addlinespace
Dum07t10       &    0.000   &    0.006   &    0.012   &   -0.015   \\
               &  (0.002)   &  (0.011)   &  (0.009)   &  (0.018)   \\
\addlinespace
Ln(Num of HH, 99) x DumD00t06&            &    0.001*  &   -0.003*  &   -0.001   \\
               &            &  (0.000)   &  (0.002)   &  (0.002)   \\
\addlinespace
Ln(Num of HH, 99) x DumD07t10&            &   -0.001***&    0.001   &   -0.001   \\
               &            &  (0.000)   &  (0.002)   &  (0.002)   \\
\addlinespace
Ln(HH Income, 99) x DumD00t06&            &   -0.001   &   -0.000   &   -0.002   \\
               &            &  (0.001)   &  (0.001)   &  (0.001)   \\
\addlinespace
Ln(HH Income, 99) x DumD07t10&            &    0.000   &    0.000   &    0.003   \\
               &            &  (0.001)   &  (0.001)   &  (0.002)   \\
\addlinespace
Ratio of Labor Force (1999) x DumD00t06&            &   -0.006** &   -0.005   &   -0.009*  \\
               &            &  (0.003)   &  (0.004)   &  (0.005)   \\
\addlinespace
Ratio of Labor Force (1999) x DumD07t10&            &    0.000   &   -0.003   &    0.000   \\
               &            &  (0.004)   &  (0.007)   &  (0.007)   \\
\addlinespace
Ln(Num of HU, 99) x DumD00t06&            &            &    0.003** &    0.002   \\
               &            &            &  (0.002)   &  (0.002)   \\
\addlinespace
Ln(Num of HU, 99) x DumD07t10&            &            &   -0.002   &   -0.001   \\
               &            &            &  (0.002)   &  (0.002)   \\
\addlinespace
Housing supply elasticity x DumD00t06&            &            &    0.000   &    0.000   \\
               &            &            &  (0.000)   &  (0.000)   \\
\addlinespace
Housing supply elasticity x DumD07t10&            &            &   -0.000   &   -0.000   \\
               &            &            &  (0.000)   &  (0.000)   \\
\addlinespace
House Vacancy Rate (1999) x DumD00t06&            &            &   -0.002   &   -0.001   \\
               &            &            &  (0.005)   &  (0.004)   \\
\addlinespace
House Vacancy Rate (1999) x DumD07t10&            &            &   -0.003   &   -0.003   \\
               &            &            &  (0.006)   &  (0.005)   \\
\addlinespace
Ratio of Renters (1999) x DumD00t06&            &            &    0.002   &    0.004   \\
               &            &            &  (0.004)   &  (0.005)   \\
\addlinespace
Ratio of Renters (1999) x DumD07t10&            &            &   -0.000   &    0.001   \\
               &            &            &  (0.005)   &  (0.006)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x DumD00t06&            &            &            &    0.007*  \\
               &            &            &            &  (0.004)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x DumD07t10&            &            &            &   -0.010** \\
               &            &            &            &  (0.005)   \\
\addlinespace
Ratio of White Race (1999) x DumD00t06&            &            &            &    0.002   \\
               &            &            &            &  (0.001)   \\
\addlinespace
Ratio of White Race (1999) x DumD07t10&            &            &            &    0.001   \\
               &            &            &            &  (0.002)   \\
\addlinespace
Ratio of Immigration (90-00) x DumD00t06&            &            &            &   -0.011   \\
               &            &            &            &  (0.012)   \\
\addlinespace
Ratio of Immigration (90-00) x DumD07t10&            &            &            &    0.011   \\
               &            &            &            &  (0.015)   \\
\midrule
Obs            &     1530   &     1530   &     1368   &     1368   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   \\
KP F-Stat (99-05, non-stack sample)       &    8.888   &    11.69   &    5.655   &    7.386   \\
MOP F-Stat (99-05, non-stack sample)  &    8.363   &    11.32   &    5.309   &    7.208   \\
CoefEqual\_Chi2  &    6.148   &    6.467   &    3.477   &    5.416   \\
CoefEqual\_PValue  &    0.013   &    0.011   &    0.062   &    0.020   \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}

==> Table_HH/table_ComConstEmp.D00t06vsD07t10.NEP.D99t05.2SLS.tex <==
%-----------------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_ComConstEmp.D00t06vsD07t10.NEP.D99t05.2SLS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Stacked Regression of Commercial Construction Employment Growth in Boom (00-06) and Bust (07-10) Periods on Net Export Growth (99-05)} \smallskip \newline
{\scriptsize
This table reports 2SLS regression $\triangle_{00,06} \& \triangle_{07,10} ComConstEmpShr_{c} = \beta_{00,06} * \triangle_{99,05} \text{NetExp}_{m} \times Dum_{00,06} + \beta_{07,10} * \triangle_{99,05} \text{NetExp}_{m} \times Dum_{07,10} + \gamma_{00,06}* \bm{Controls_{c}} \times Dum_{00,06} + \gamma_{07,10}* \bm{Controls_{c}} \times Dum_{07,10} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{00,06} \& \triangle_{07,10} ComConstEmpShr_{c}$ is the change of the commercial construction employment share in working-age population at county $c$ 00-06 and 07-10. The key independent variable $\triangle_{99,05} \text{NetExp}_{m}$ is the growth rate of net export growth in metropolitan area $m$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in the period start year 1999. We use the gravity model-based instrumental variable $\triangle_{99,05}\text{givNetExp}_{m}$ as the IV for $\triangle_{99,05}\text{NetExp}_{m}$. Regression is weighted by the natural logarithm of housing units in 1999.  For the first-stage F-test of two non-stacked samples, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
\smallskip
} % end of small font size
} % end of caption
\label{table_ComConstEmp.D00t06vsD07t10.NEP.D99t05.2SLS}

\vspace{-2mm}

\resizebox{0.55\columnwidth}{!}{%
\begin{tabular}{l*{4}{c}}
\toprule
\textbf{TSLS estimates}            &\multicolumn{4}{c}{Tradable Employment Growth (00-06 and 07-10, An)} \\
            \cmidrule{2-5} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
            
\midrule
Net Export Growth (99-05, An) x Dum00t06&    0.684   &    0.605   &    0.036   &    0.011   \\
               &  (1.519)   &  (1.564)   &  (1.579)   &  (1.529)   \\
\addlinespace
Net Export Growth (99-05, An) x Dum07t10&    0.076   &    0.592   &    0.124   &   -0.161   \\
               &  (1.633)   &  (1.723)   &  (2.046)   &  (2.028)   \\
\addlinespace
Dum00t06       &    0.004   &   -0.155** &   -0.160*  &   -0.230   \\
               &  (0.004)   &  (0.068)   &  (0.085)   &  (0.143)   \\
\addlinespace
Dum07t10       &   -0.015***&    0.492***&    0.671***&    0.619** \\
               &  (0.005)   &  (0.130)   &  (0.148)   &  (0.289)   \\
\addlinespace
Ln(Num of HH, 99) x DumD00t06&            &   -0.002   &   -0.023   &   -0.031   \\
               &            &  (0.002)   &  (0.028)   &  (0.029)   \\
\addlinespace
Ln(Num of HH, 99) x DumD07t10&            &    0.004   &    0.055** &    0.054*  \\
               &            &  (0.003)   &  (0.028)   &  (0.032)   \\
\addlinespace
Ln(HH Income, 99) x DumD00t06&            &    0.019** &    0.014   &    0.022   \\
               &            &  (0.008)   &  (0.009)   &  (0.014)   \\
\addlinespace
Ln(HH Income, 99) x DumD07t10&            &   -0.054***&   -0.066***&   -0.059** \\
               &            &  (0.014)   &  (0.016)   &  (0.028)   \\
\addlinespace
Ratio of Labor Force (1999) x DumD00t06&            &   -0.038   &    0.004   &    0.020   \\
               &            &  (0.028)   &  (0.034)   &  (0.037)   \\
\addlinespace
Ratio of Labor Force (1999) x DumD07t10&            &    0.049   &   -0.011   &   -0.011   \\
               &            &  (0.065)   &  (0.063)   &  (0.065)   \\
\addlinespace
Ln(Num of HU, 99) x DumD00t06&            &            &    0.023   &    0.031   \\
               &            &            &  (0.028)   &  (0.029)   \\
\addlinespace
Ln(Num of HU, 99) x DumD07t10&            &            &   -0.052*  &   -0.051*  \\
               &            &            &  (0.027)   &  (0.031)   \\
\addlinespace
Housing supply elasticity x DumD00t06&            &            &   -0.001   &   -0.001   \\
               &            &            &  (0.002)   &  (0.002)   \\
\addlinespace
Housing supply elasticity x DumD07t10&            &            &    0.000   &   -0.000   \\
               &            &            &  (0.003)   &  (0.003)   \\
\addlinespace
House Vacancy Rate (1999) x DumD00t06&            &            &    0.057   &    0.051   \\
               &            &            &  (0.047)   &  (0.049)   \\
\addlinespace
House Vacancy Rate (1999) x DumD07t10&            &            &   -0.027   &   -0.028   \\
               &            &            &  (0.075)   &  (0.077)   \\
\addlinespace
Ratio of Renters (1999) x DumD00t06&            &            &   -0.022   &   -0.030   \\
               &            &            &  (0.022)   &  (0.029)   \\
\addlinespace
Ratio of Renters (1999) x DumD07t10&            &            &   -0.018   &   -0.015   \\
               &            &            &  (0.035)   &  (0.048)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x DumD00t06&            &            &            &   -0.031   \\
               &            &            &            &  (0.037)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x DumD07t10&            &            &            &    0.000   \\
               &            &            &            &  (0.073)   \\
\addlinespace
Ratio of White Race (1999) x DumD00t06&            &            &            &   -0.011   \\
               &            &            &            &  (0.013)   \\
\addlinespace
Ratio of White Race (1999) x DumD07t10&            &            &            &   -0.027   \\
               &            &            &            &  (0.025)   \\
\addlinespace
Ratio of Immigration (90-00) x DumD00t06&            &            &            &    0.048   \\
               &            &            &            &  (0.066)   \\
\addlinespace
Ratio of Immigration (90-00) x DumD07t10&            &            &            &   -0.160   \\
               &            &            &            &  (0.119)   \\
\midrule
Obs            &     1520   &     1520   &     1340   &     1340   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   \\
KP F-Stat (99-05, non-stack sample)  &    22.58   &    22.23   &    15.88   &    17.18   \\
MOP F-Stat (99-05, non-stack sample)  &    22.01   &    21.62   &    15.43   &    16.74   \\
CoefEqual\_Chi2  &    0.048   &    0.000   &    0.001   &    0.003   \\
CoefEqual\_PValue  &    0.826   &    0.997   &    0.979   &    0.958   \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}

==> Table_HH/table_HHDTI.D99t05vsD08t14.GSEM.2SLS.tex <==
%-----------------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_HHDTI.D99t05vsD08t14.GSEM.2SLS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Stacked Regression of Household Leverage in Boom (99-05) and Bust (08-14) Periods on GSEM Growth (99-05)} \smallskip \newline
{\scriptsize
This table reports 2SLS regression $\triangle_{99,05} \& \triangle_{08,14} HHDTI_{c} = \beta_{99,05} * \triangle_{99,05} Ln(GSEM_{c}) \times Dum_{99,05} + \beta_{08,14} * \triangle_{99,05} Ln(GSEM_{c}) \times Dum_{08,14} + \gamma_{99,05}* \bm{Controls_{c}} \times Dum_{99,05} + \gamma_{08,14}* \bm{Controls_{c}} \times Dum_{08,14} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{99,05} \& \triangle_{08,14} HHDTI_{c}$ is the stacked increase in household leverage (debt-to-income ratio) at county $c$ 99-05 and 08-14. The key independent variable $\triangle_{99,05} Ln(GSEM_{c})$ is the growth rate of the dollar amount (deflated to 2007 USD) of government-sponsored enterprise mortgages (non-jumbo) at county $c$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in the period start year 1999. We use the gravity model-based instrumental variable $\triangle_{99,05}\text{givNetExp}_{m}$ as the IV for $\triangle_{99,05}Ln(GSEM_{c})$. Regression is weighted by the natural logarithm of housing units in 1999.  For the first-stage F-test of two non-stacked samples, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
\smallskip
} % end of small font size
} % end of caption
\label{table_HHDTI.D99t05vsD08t14.GSEM.2SLS}

\vspace{-2mm}

\resizebox{0.55\columnwidth}{!}{%
\begin{tabular}{l*{5}{c}}
\toprule
\textbf{TSLS estimates}            &\multicolumn{5}{c}{Household Leverage Increase (99-05 and 07-09, Annualized )} \\
            \cmidrule{2-6} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
            
\midrule
GSEM Growth (99-05, An) x Dum99t05&    5.646   &    2.299*  &    2.878   &    3.143   &    4.687   \\
               &  (8.229)   &  (1.300)   &  (2.509)   &  (2.380)   &  (5.481)   \\
\addlinespace
GSEM Growth (99-05, An) x Dum08t14&   -7.968   &   -3.093*  &   -4.262   &   -4.189   &   -6.493   \\
               & (11.439)   &  (1.730)   &  (3.724)   &  (3.283)   &  (7.787)   \\
\addlinespace
Dum99t05       &   -0.089   &   -3.245** &   -2.588   &   -4.467   &   -6.771   \\
               &  (0.336)   &  (1.478)   &  (2.242)   &  (3.391)   &  (7.831)   \\
\addlinespace
Dum08t14       &    0.244   &    4.042** &    3.976   &    6.711   &   10.095   \\
               &  (0.466)   &  (1.935)   &  (3.314)   &  (4.564)   & (10.929)   \\
\addlinespace
Ln(Num of HH, 99) x Dum99t05&            &    0.002   &    0.021   &   -0.198   &   -0.263   \\
               &            &  (0.021)   &  (0.113)   &  (0.169)   &  (0.294)   \\
\addlinespace
Ln(Num of HH, 99) x Dum08t14&            &   -0.039   &    0.050   &    0.323   &    0.398   \\
               &            &  (0.027)   &  (0.188)   &  (0.251)   &  (0.432)   \\
\addlinespace
Ln(HH Income, 99) x Dum99t05&            &    0.270***&    0.187   &    0.381   &    0.559   \\
               &            &  (0.105)   &  (0.148)   &  (0.275)   &  (0.610)   \\
\addlinespace
Ln(HH Income, 99) x Dum08t14&            &   -0.303** &   -0.254   &   -0.548   &   -0.809   \\
               &            &  (0.135)   &  (0.219)   &  (0.366)   &  (0.849)   \\
\addlinespace
Ratio of Labor Force (1999) x Dum99t05&            &    0.572   &    0.901   &    1.454*  &    2.011   \\
               &            &  (0.350)   &  (0.628)   &  (0.820)   &  (1.946)   \\
\addlinespace
Ratio of Labor Force (1999) x Dum08t14&            &   -0.490   &   -1.014   &   -1.626   &   -2.442   \\
               &            &  (0.485)   &  (0.945)   &  (1.141)   &  (2.780)   \\
\addlinespace
Ln(Num of HU, 99) x Dum99t05&            &            &   -0.005   &    0.205   &    0.289   \\
               &            &            &  (0.123)   &  (0.190)   &  (0.353)   \\
\addlinespace
Ln(Num of HU, 99) x Dum08t14&            &            &   -0.107   &   -0.367   &   -0.474   \\
               &            &            &  (0.202)   &  (0.277)   &  (0.513)   \\
\addlinespace
Housing supply elasticity x Dum99t05&            &            &   -0.023** &   -0.020*  &   -0.022   \\
               &            &            &  (0.011)   &  (0.010)   &  (0.016)   \\
\addlinespace
Housing supply elasticity x Dum08t14&            &            &    0.019   &    0.016   &    0.017   \\
               &            &            &  (0.016)   &  (0.014)   &  (0.023)   \\
\addlinespace
House Vacancy Rate (1999) x Dum99t05&            &            &   -0.339   &   -0.552   &   -0.865   \\
               &            &            &  (0.654)   &  (0.701)   &  (1.396)   \\
\addlinespace
House Vacancy Rate (1999) x Dum08t14&            &            &    0.730   &    0.890   &    1.380   \\
               &            &            &  (0.977)   &  (0.987)   &  (2.021)   \\
\addlinespace
Ratio of Renters (1999) x Dum99t05&            &            &   -0.254   &   -0.629***&   -0.409   \\
               &            &            &  (0.178)   &  (0.191)   &  (0.295)   \\
\addlinespace
Ratio of Renters (1999) x Dum08t14&            &            &    0.123   &    0.521*  &    0.208   \\
               &            &            &  (0.291)   &  (0.276)   &  (0.444)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x Dum99t05&            &            &            &   -0.880   &   -0.623   \\
               &            &            &            &  (0.582)   &  (0.601)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x Dum08t14&            &            &            &    1.273*  &    0.825   \\
               &            &            &            &  (0.773)   &  (0.829)   \\
\addlinespace
Ratio of White Race (1999) x Dum99t05&            &            &            &   -0.294   &   -0.318   \\
               &            &            &            &  (0.222)   &  (0.372)   \\
\addlinespace
Ratio of White Race (1999) x Dum08t14&            &            &            &    0.423   &    0.453   \\
               &            &            &            &  (0.301)   &  (0.530)   \\
\addlinespace
Ratio of Immigration (90-00) x Dum99t05&            &            &            &    2.351** &    2.445   \\
               &            &            &            &  (1.118)   &  (1.738)   \\
\addlinespace
Ratio of Immigration (90-00) x Dum08t14&            &            &            &   -2.389   &   -2.426   \\
               &            &            &            &  (1.542)   &  (2.401)   \\
\addlinespace
Ratio of Art, Enter, and Recre Emp (1999) x Dum99t05&            &            &            &            &   -6.075   \\
               &            &            &            &            &  (7.106)   \\
\addlinespace
Ratio of Art, Enter, and Recre Emp (1999) x Dum08t14&            &            &            &            &    8.300   \\
               &            &            &            &            & (10.041)   \\
\addlinespace
Ratio of Health Emp (1999) x Dum99t05&            &            &            &            &   -3.180   \\
               &            &            &            &            &  (3.967)   \\
\addlinespace
Ratio of Health Emp (1999) x Dum08t14&            &            &            &            &    5.576   \\
               &            &            &            &            &  (5.872)   \\
\addlinespace
Ratio of Tradable Service Emp (1999) x Dum99t05&            &            &            &            &   -1.566   \\
               &            &            &            &            &  (2.765)   \\
\addlinespace
Ratio of Tradable Service Emp (1999) x Dum08t14&            &            &            &            &    2.565   \\
               &            &            &            &            &  (4.041)   \\
\addlinespace
Ratio of College Students (1999) x Dum99t05&            &            &            &            &   -0.933   \\
               &            &            &            &            &  (0.941)   \\
\addlinespace
Ratio of College Students (1999) x Dum08t14&            &            &            &            &    0.943   \\
               &            &            &            &            &  (1.402)   \\
\midrule
Obs            &     1584   &     1584   &     1402   &     1402   &     1402   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   \\
KP F-Stat (99-05, non-stack sample)       &    0.530   &    4.246   &    1.643   &    1.962   &    0.773   \\
MOP F-Stat (99-05, non-stack sample)  &    0.534   &    4.247   &    1.639   &    1.981   &    0.777   \\
CoefEqual\_Chi2 &    0.484   &    3.324   &    1.366   &    1.745   &    0.722   \\
CoefEqual\_PValue &    0.487   &    0.068   &    0.242   &    0.187   &    0.395   \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}

==> Table_HH/table_HHDTI.D99t05vsD08t14.PLMNJ.2SLS.tex <==
%-----------------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_HHDTI.D99t05vsD08t14.PLMNJ.2SLS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Stacked Regression of Household Leverage in Boom (99-05) and Bust (08-14) Periods on PLMNJ Growth (99-05)} \smallskip \newline
{\scriptsize
This table reports 2SLS regression $\triangle_{99,05} \& \triangle_{08,14} HHDTI_{c} = \beta_{99,05} * \triangle_{99,05} Ln(PLMNJ_{c}) \times Dum_{99,05} + \beta_{08,14} * \triangle_{99,05} Ln(PLMNJ_{c}) \times Dum_{08,14} + \gamma_{99,05}* \bm{Controls_{c}} \times Dum_{99,05} + \gamma_{08,14}* \bm{Controls_{c}} \times Dum_{08,14} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{99,05} \& \triangle_{08,14} HHDTI_{c}$ is the stacked increase in household leverage (debt-to-income ratio) at county $c$ 99-05 and 08-14. The key independent variable $\triangle_{99,05} Ln(PLMNJ_{c})$ is the growth rate of the dollar amount (deflated to 2007 USD) of private-label mortgages (non-jumbo) at county $c$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in the period start year 1999. We use the gravity model-based instrumental variable $\triangle_{99,05}\text{givNetExp}_{m}$ as the IV for $\triangle_{99,05}Ln(PLMNJ_{c})$. Regression is weighted by the natural logarithm of housing units in 1999.  For the first-stage F-test of two non-stacked samples, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
\smallskip
} % end of small font size
} % end of caption
\label{table_HHDTI.D99t05vsD08t14.PLMNJ.2SLS}

\vspace{-2mm}

\resizebox{0.55\columnwidth}{!}{%
\begin{tabular}{l*{5}{c}}
\toprule
\textbf{TSLS estimates}            &\multicolumn{5}{c}{Household Leverage Increase (99-05 and 07-09, Annualized )} \\
            \cmidrule{2-6} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
            
\midrule
PLMNJ Growth (99-05, An) x Dum99t05&    0.779***&    0.796***&    0.793** &    0.912***&    0.940***\\
               &  (0.246)   &  (0.258)   &  (0.312)   &  (0.305)   &  (0.342)   \\
\addlinespace
PLMNJ Growth (99-05, An) x Dum08t14&   -1.099***&   -1.071***&   -1.174***&   -1.216***&   -1.302***\\
               &  (0.289)   &  (0.323)   &  (0.410)   &  (0.401)   &  (0.433)   \\
\addlinespace
Dum99t05       &    0.013   &   -0.919***&   -0.418   &   -0.334   &   -0.311   \\
               &  (0.041)   &  (0.258)   &  (0.338)   &  (0.566)   &  (0.549)   \\
\addlinespace
Dum08t14       &    0.100** &    0.913***&    0.762** &    1.203** &    1.146*  \\
               &  (0.048)   &  (0.275)   &  (0.371)   &  (0.571)   &  (0.607)   \\
\addlinespace
Ln(Num of HH, 99) x Dum99t05&            &   -0.038***&    0.034   &   -0.031   &   -0.035   \\
               &            &  (0.008)   &  (0.062)   &  (0.056)   &  (0.057)   \\
\addlinespace
Ln(Num of HH, 99) x Dum08t14&            &    0.015** &    0.030   &    0.101   &    0.082   \\
               &            &  (0.006)   &  (0.067)   &  (0.067)   &  (0.068)   \\
\addlinespace
Ln(HH Income, 99) x Dum99t05&            &    0.119***&    0.067*  &    0.065   &    0.064   \\
               &            &  (0.031)   &  (0.040)   &  (0.062)   &  (0.060)   \\
\addlinespace
Ln(HH Income, 99) x Dum08t14&            &   -0.100***&   -0.077** &   -0.127** &   -0.123** \\
               &            &  (0.029)   &  (0.039)   &  (0.055)   &  (0.057)   \\
\addlinespace
Ratio of Labor Force (1999) x Dum99t05&            &    0.097   &    0.179   &    0.309*  &    0.290*  \\
               &            &  (0.122)   &  (0.192)   &  (0.167)   &  (0.160)   \\
\addlinespace
Ratio of Labor Force (1999) x Dum08t14&            &    0.149   &    0.055   &   -0.100   &   -0.058   \\
               &            &  (0.119)   &  (0.149)   &  (0.148)   &  (0.149)   \\
\addlinespace
Ln(Num of HU, 99) x Dum99t05&            &            &   -0.064   &   -0.006   &   -0.006   \\
               &            &            &  (0.067)   &  (0.061)   &  (0.062)   \\
\addlinespace
Ln(Num of HU, 99) x Dum08t14&            &            &   -0.019   &   -0.085   &   -0.065   \\
               &            &            &  (0.067)   &  (0.067)   &  (0.069)   \\
\addlinespace
Housing supply elasticity x Dum99t05&            &            &   -0.007   &   -0.004   &   -0.005   \\
               &            &            &  (0.006)   &  (0.006)   &  (0.006)   \\
\addlinespace
Housing supply elasticity x Dum08t14&            &            &   -0.004   &   -0.006   &   -0.007   \\
               &            &            &  (0.007)   &  (0.007)   &  (0.007)   \\
\addlinespace
House Vacancy Rate (1999) x Dum99t05&            &            &    0.140   &    0.055   &    0.125   \\
               &            &            &  (0.195)   &  (0.190)   &  (0.190)   \\
\addlinespace
House Vacancy Rate (1999) x Dum08t14&            &            &    0.021   &    0.082   &    0.009   \\
               &            &            &  (0.184)   &  (0.188)   &  (0.174)   \\
\addlinespace
Ratio of Renters (1999) x Dum99t05&            &            &   -0.260** &   -0.438***&   -0.358***\\
               &            &            &  (0.128)   &  (0.118)   &  (0.109)   \\
\addlinespace
Ratio of Renters (1999) x Dum08t14&            &            &    0.132   &    0.266***&    0.137   \\
               &            &            &  (0.109)   &  (0.098)   &  (0.109)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x Dum99t05&            &            &            &   -0.120   &   -0.147   \\
               &            &            &            &  (0.141)   &  (0.180)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x Dum08t14&            &            &            &    0.261*  &    0.166   \\
               &            &            &            &  (0.157)   &  (0.187)   \\
\addlinespace
Ratio of White Race (1999) x Dum99t05&            &            &            &   -0.043   &   -0.023   \\
               &            &            &            &  (0.074)   &  (0.074)   \\
\addlinespace
Ratio of White Race (1999) x Dum08t14&            &            &            &    0.087   &    0.044   \\
               &            &            &            &  (0.055)   &  (0.055)   \\
\addlinespace
Ratio of Immigration (90-00) x Dum99t05&            &            &            &    1.199***&    1.133***\\
               &            &            &            &  (0.287)   &  (0.305)   \\
\addlinespace
Ratio of Immigration (90-00) x Dum08t14&            &            &            &   -0.854***&   -0.608*  \\
               &            &            &            &  (0.301)   &  (0.319)   \\
\addlinespace
Ratio of Art, Enter, and Recre Emp (1999) x Dum99t05&            &            &            &            &   -2.183** \\
               &            &            &            &            &  (0.909)   \\
\addlinespace
Ratio of Art, Enter, and Recre Emp (1999) x Dum08t14&            &            &            &            &    2.909** \\
               &            &            &            &            &  (1.369)   \\
\addlinespace
Ratio of Health Emp (1999) x Dum99t05&            &            &            &            &   -0.127   \\
               &            &            &            &            &  (0.687)   \\
\addlinespace
Ratio of Health Emp (1999) x Dum08t14&            &            &            &            &    1.347*  \\
               &            &            &            &            &  (0.689)   \\
\addlinespace
Ratio of Tradable Service Emp (1999) x Dum99t05&            &            &            &            &    0.409   \\
               &            &            &            &            &  (0.449)   \\
\addlinespace
Ratio of Tradable Service Emp (1999) x Dum08t14&            &            &            &            &   -0.171   \\
               &            &            &            &            &  (0.481)   \\
\addlinespace
Ratio of College Students (1999) x Dum99t05&            &            &            &            &   -0.423** \\
               &            &            &            &            &  (0.213)   \\
\addlinespace
Ratio of College Students (1999) x Dum08t14&            &            &            &            &    0.236   \\
               &            &            &            &            &  (0.250)   \\

\midrule
Obs            &     1584   &     1584   &     1402   &     1402   &     1402   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   \\
KP F-Stat (99-05, non-stack sample)       &    23.43   &    21.04   &    13.97   &    11.74   &    11.43   \\
MOP F-Stat (99-05, non-stack sample)  &    22.30   &    20.29   &    14.03   &    11.80   &    11.37   \\
CoefEqual\_Chi2 &   15.947   &   12.191   &    9.512   &   11.555   &   10.476   \\
CoefEqual\_PValue &    0.000   &    0.000   &    0.002   &    0.001   &    0.001   \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}

==> Table_HH/table_HPI.D99t05vsD07t09.HHDTI.2SLS.tex <==
%-----------------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_HPI.D99t05vsD07t09.HHDTI.2SLS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Stacked Regression of Housing Price Growth in Boom (99-05) and Bust (07-09) Periods on Household Leverage Increase (99-05)} \smallskip \newline
{\scriptsize
This table reports 2SLS regression $\triangle_{99,05} \& \triangle_{07,09} Ln(HPI_{c}) = \beta_{99,05} * \triangle_{99,05} HHDTI_{c} \times Dum_{99,05} + \beta_{07,09} * \triangle_{99,05} HHDTI_{c} \times Dum_{07,09} + \gamma_{99,05}* \bm{Controls_{c}} \times Dum_{99,05} + \gamma_{07,09}* \bm{Controls_{c}} \times Dum_{07,09} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{99,05} \& \triangle_{07,09} Ln(HPI_{c})$ is the stacked growth rate of the house price index (deflated to 2007) at county $c$ 99-05 and 07-09. The key independent variable $\triangle_{99,05} HHDTI_{c}$ is the rise in household leverage (debt-to-income ratio) at county $c$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in the period start year 1999. We use the gravity model-based instrumental variable $\triangle_{99,05}\text{givNetExp}_{m}$ as the IV for $\triangle_{99,05}HHDTI_{c}$. Regression is weighted by the natural logarithm of housing units in 1999. For the first-stage F-test of two non-stacked samples, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
\smallskip
} % end of small font size
} % end of caption
\label{table_HPI.D99t05vsD07t09.HHDTI.2SLS}

\vspace{-2mm}

\resizebox{0.55\columnwidth}{!}{%
\begin{tabular}{l*{5}{c}}
\toprule
\textbf{TSLS estimates}            &\multicolumn{5}{c}{Housing Price Growth (99-05 and 07-09, Annualized )} \\
            \cmidrule{2-6} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
            
\midrule
HH Debt-to-Income Rise (99-05, An) x Dum99t05&    0.630***&    0.534***&    0.479** &    0.455***&    0.445** \\
               &  (0.174)   &  (0.173)   &  (0.195)   &  (0.161)   &  (0.175)   \\
\addlinespace
HH Debt-to-Income Rise (99-05, An) x Dum07t09&   -0.378***&   -0.337***&   -0.329***&   -0.296***&   -0.304***\\
               &  (0.104)   &  (0.091)   &  (0.116)   &  (0.091)   &  (0.103)   \\
\addlinespace
Dum99t05       &   -0.053** &   -0.044   &   -0.316** &   -0.104   &   -0.141   \\
               &  (0.024)   &  (0.177)   &  (0.140)   &  (0.208)   &  (0.198)   \\
\addlinespace
Dum07t09       &    0.037** &   -0.119   &   -0.002   &    0.143   &    0.161   \\
               &  (0.015)   &  (0.084)   &  (0.083)   &  (0.153)   &  (0.143)   \\
\addlinespace
Ln(Num of HH, 99) x DumD99t05&            &    0.024***&    0.003   &    0.031   &    0.032   \\
               &            &  (0.006)   &  (0.034)   &  (0.029)   &  (0.029)   \\
\addlinespace
Ln(Num of HH, 99) x DumD07t09&            &   -0.016***&   -0.004   &   -0.012   &   -0.014   \\
               &            &  (0.003)   &  (0.024)   &  (0.020)   &  (0.021)   \\
\addlinespace
Ln(HH Income, 99) x DumD99t05&            &   -0.011   &    0.023   &    0.003   &    0.006   \\
               &            &  (0.024)   &  (0.019)   &  (0.025)   &  (0.024)   \\
\addlinespace
Ln(HH Income, 99) x DumD07t09&            &    0.023** &    0.008   &   -0.006   &   -0.007   \\
               &            &  (0.011)   &  (0.011)   &  (0.017)   &  (0.016)   \\
\addlinespace
Ratio of Labor Force (1999) x DumD99t05&            &   -0.214***&   -0.243***&   -0.296***&   -0.283***\\
               &            &  (0.062)   &  (0.079)   &  (0.086)   &  (0.088)   \\
\addlinespace
Ratio of Labor Force (1999) x DumD07t09&            &    0.122***&    0.161** &    0.165***&    0.160** \\
               &            &  (0.040)   &  (0.067)   &  (0.063)   &  (0.063)   \\
\addlinespace
Ln(Num of HU, 99) x DumD99t05&            &            &    0.008   &   -0.019   &   -0.020   \\
               &            &            &  (0.038)   &  (0.031)   &  (0.031)   \\
\addlinespace
Ln(Num of HU, 99) x DumD07t09&            &            &   -0.008   &   -0.001   &    0.000   \\
               &            &            &  (0.026)   &  (0.021)   &  (0.022)   \\
\addlinespace
Housing supply elasticity x DumD99t05&            &            &   -0.002   &   -0.003   &   -0.003   \\
               &            &            &  (0.004)   &  (0.003)   &  (0.003)   \\
\addlinespace
Housing supply elasticity x DumD07t09&            &            &   -0.001   &   -0.001   &   -0.001   \\
               &            &            &  (0.002)   &  (0.002)   &  (0.002)   \\
\addlinespace
House Vacancy Rate (1999) x DumD99t05&            &            &    0.008   &    0.033   &    0.020   \\
               &            &            &  (0.112)   &  (0.091)   &  (0.097)   \\
\addlinespace
House Vacancy Rate (1999) x DumD07t09&            &            &    0.053   &    0.032   &    0.067   \\
               &            &            &  (0.071)   &  (0.058)   &  (0.062)   \\
\addlinespace
Ratio of Renters (1999) x DumD99t05&            &            &    0.258***&    0.282***&    0.235** \\
               &            &            &  (0.088)   &  (0.098)   &  (0.100)   \\
\addlinespace
Ratio of Renters (1999) x DumD07t09&            &            &   -0.101*  &   -0.124** &   -0.110*  \\
               &            &            &  (0.057)   &  (0.058)   &  (0.058)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x DumD99t05&            &            &            &    0.114*  &    0.091   \\
               &            &            &            &  (0.065)   &  (0.079)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x DumD07t09&            &            &            &    0.023   &   -0.024   \\
               &            &            &            &  (0.047)   &  (0.067)   \\
\addlinespace
Ratio of White Race (1999) x DumD99t05&            &            &            &    0.015   &    0.001   \\
               &            &            &            &  (0.031)   &  (0.031)   \\
\addlinespace
Ratio of White Race (1999) x DumD07t09&            &            &            &   -0.003   &   -0.001   \\
               &            &            &            &  (0.018)   &  (0.018)   \\
\addlinespace
Ratio of Immigration (90-00) x DumD99t05&            &            &            &   -0.323   &   -0.235   \\
               &            &            &            &  (0.236)   &  (0.259)   \\
\addlinespace
Ratio of Immigration (90-00) x DumD07t09&            &            &            &    0.165   &    0.172   \\
               &            &            &            &  (0.131)   &  (0.155)   \\
\addlinespace
Ratio of Art, Enter, and Recre Emp (1999) x DumD99t05&            &            &            &            &    0.714***\\
               &            &            &            &            &  (0.200)   \\
\addlinespace
Ratio of Art, Enter, and Recre Emp (1999) x DumD07t09&            &            &            &            &   -0.689***\\
               &            &            &            &            &  (0.171)   \\
\addlinespace
Ratio of Health Emp (1999) x DumD99t05&            &            &            &            &    0.377   \\
               &            &            &            &            &  (0.235)   \\
\addlinespace
Ratio of Health Emp (1999) x DumD07t09&            &            &            &            &    0.101   \\
               &            &            &            &            &  (0.194)   \\
\addlinespace
Ratio of Tradable Service Emp (1999) x DumD99t05&            &            &            &            &   -0.090   \\
               &            &            &            &            &  (0.172)   \\
\addlinespace
Ratio of Tradable Service Emp (1999) x DumD07t09&            &            &            &            &    0.258*  \\
               &            &            &            &            &  (0.132)   \\
\addlinespace
Ratio of College Students (1999) x DumD99t05&            &            &            &            &    0.145   \\
               &            &            &            &            &  (0.122)   \\
\addlinespace
Ratio of College Students (1999) x DumD07t09&            &            &            &            &   -0.098   \\
               &            &            &            &            &  (0.068)   \\
\midrule
Obs            &     1572   &     1572   &     1390   &     1390   &     1390   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   \\
KP F-Stat (99-05, non-stack sample)       &    10.88   &    13.23   &    7.776   &    10.19   &    8.736   \\
MOP F-Stat (99-05, non-stack sample)  &    9.760   &    12.36   &    7.059   &    9.542   &    7.959   \\
CoefEqual\_Chi2 &   14.521   &   12.057   &    7.399   &    9.896   &    8.301   \\
CoefEqual\_PValue &    0.000   &    0.001   &    0.007   &    0.002   &    0.004   \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}

==> Table_HH/table_Permit.D99t05vsD05t09.HHDTI.2SLS.tex <==
%-----------------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_Permit.D99t05vsD05t09.HHDTI.2SLS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Stacked Regression of Residential Construction Permit Value Growth in Boom (99-05) and Bust (05-09) Periods on Household Leverage Rise (99-05)} \smallskip \newline
{\scriptsize
This table reports 2SLS regression $\triangle_{99,05} \& \triangle_{05,09} Ln(\text{PermitValue}_{c}) = \beta_{99,05} * \triangle_{99,05} HHDTI_{c} \times Dum_{99,05} + \beta_{05,09} * \triangle_{99,05} HHDTI_{c} \times Dum_{05,09} + \gamma_{99,05}* \bm{Controls_{c}} \times Dum_{99,05} + \gamma_{05,09}* \bm{Controls_{c}} \times Dum_{05,09} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{99,05} \& \triangle_{05,09} Ln(\text{PermitValue}_{c})$ is the stacked growth rate of the residential construction permit value (deflated to 2007) at county $c$ 99-05 and 05-09. The key independent variable $\triangle_{99,05} HHDTI_{c}$ is the rise in household leverage (debt-to-income ratio) at county $c$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in the period start year 1999. We use the gravity model-based instrumental variable $\triangle_{99,05}\text{givNetExp}_{m}$ as the IV for $\triangle_{99,05}HHDTI_{c}$. Regression is weighted by the natural logarithm of housing units in 1999. For the first-stage F-test of two non-stacked samples, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
\smallskip
} % end of small font size
} % end of caption
\label{table_Permit.D99t05vsD05t09.HHDTI.2SLS}

\vspace{-2mm}

\resizebox{0.55\columnwidth}{!}{%
\begin{tabular}{l*{5}{c}}
\toprule
\textbf{TSLS estimates}            &\multicolumn{5}{c}{Residential Permit Value Growth (99-05 and 05-09, Annualized)} \\
            \cmidrule{2-6} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
            
\midrule
HH Debt-to-Income Rise (99-05, An) x Dum99t05&    0.919** &    1.080***&    0.853*  &    0.798** &    0.749*  \\
               &  (0.372)   &  (0.390)   &  (0.449)   &  (0.389)   &  (0.391)   \\
\addlinespace
HH Debt-to-Income Rise (99-05, An) x Dum05t09&   -2.061***&   -1.844***&   -2.098** &   -1.808***&   -1.839** \\
               &  (0.718)   &  (0.625)   &  (0.884)   &  (0.693)   &  (0.738)   \\
\addlinespace
Dum99t05       &   -0.067   &    1.753***&    0.919***&    1.255** &    1.335***\\
               &  (0.053)   &  (0.402)   &  (0.307)   &  (0.516)   &  (0.490)   \\
\addlinespace
Dum05t09       &    0.002   &   -0.604   &   -0.146   &    1.636   &    1.519   \\
               &  (0.102)   &  (0.719)   &  (0.640)   &  (1.124)   &  (1.134)   \\
\addlinespace
Ln(Num of HH, 99) x DumD99t05&            &    0.033***&   -0.027   &   -0.001   &    0.008   \\
               &            &  (0.013)   &  (0.069)   &  (0.061)   &  (0.063)   \\
\addlinespace
Ln(Num of HH, 99) x DumD05t09&            &   -0.069***&    0.103   &    0.061   &    0.033   \\
               &            &  (0.022)   &  (0.128)   &  (0.108)   &  (0.111)   \\
\addlinespace
Ln(HH Income, 99) x DumD99t05&            &   -0.188***&   -0.098** &   -0.124** &   -0.128** \\
               &            &  (0.054)   &  (0.039)   &  (0.058)   &  (0.055)   \\
\addlinespace
Ln(HH Income, 99) x DumD05t09&            &    0.104   &    0.062   &   -0.105   &   -0.094   \\
               &            &  (0.095)   &  (0.084)   &  (0.123)   &  (0.122)   \\
\addlinespace
Ratio of Labor Force (1999) x DumD99t05&            &   -0.287** &   -0.312*  &   -0.355*  &   -0.362*  \\
               &            &  (0.137)   &  (0.189)   &  (0.210)   &  (0.200)   \\
\addlinespace
Ratio of Labor Force (1999) x DumD05t09&            &    0.327   &    0.491   &    0.470   &    0.515   \\
               &            &  (0.243)   &  (0.455)   &  (0.444)   &  (0.437)   \\
\addlinespace
Ln(Num of HU, 99) x DumD99t05&            &            &    0.041   &    0.015   &    0.006   \\
               &            &            &  (0.074)   &  (0.063)   &  (0.063)   \\
\addlinespace
Ln(Num of HU, 99) x DumD05t09&            &            &   -0.167   &   -0.128   &   -0.108   \\
               &            &            &  (0.138)   &  (0.109)   &  (0.110)   \\
\addlinespace
Housing supply elasticity x DumD99t05&            &            &    0.006   &    0.004   &    0.004   \\
               &            &            &  (0.009)   &  (0.008)   &  (0.008)   \\
\addlinespace
Housing supply elasticity x DumD05t09&            &            &   -0.019   &   -0.013   &   -0.018   \\
               &            &            &  (0.019)   &  (0.014)   &  (0.014)   \\
\addlinespace
House Vacancy Rate (1999) x DumD99t05&            &            &    0.037   &    0.059   &    0.063   \\
               &            &            &  (0.237)   &  (0.205)   &  (0.205)   \\
\addlinespace
House Vacancy Rate (1999) x DumD05t09&            &            &    0.583   &    0.414   &    0.572   \\
               &            &            &  (0.471)   &  (0.377)   &  (0.394)   \\
\addlinespace
Ratio of Renters (1999) x DumD99t05&            &            &    0.364** &    0.350*  &    0.326*  \\
               &            &            &  (0.166)   &  (0.205)   &  (0.187)   \\
\addlinespace
Ratio of Renters (1999) x DumD05t09&            &            &   -0.424   &   -0.647*  &   -0.704*  \\
               &            &            &  (0.358)   &  (0.372)   &  (0.367)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x DumD99t05&            &            &            &    0.178   &    0.162   \\
               &            &            &            &  (0.145)   &  (0.167)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x DumD05t09&            &            &            &    0.395   &    0.020   \\
               &            &            &            &  (0.318)   &  (0.387)   \\
\addlinespace
Ratio of White Race (1999) x DumD99t05&            &            &            &   -0.045   &   -0.041   \\
               &            &            &            &  (0.059)   &  (0.058)   \\
\addlinespace
Ratio of White Race (1999) x DumD05t09&            &            &            &   -0.035   &   -0.078   \\
               &            &            &            &  (0.100)   &  (0.098)   \\
\addlinespace
Ratio of Immigration (90-00) x DumD99t05&            &            &            &   -0.555   &   -0.573   \\
               &            &            &            &  (0.515)   &  (0.503)   \\
\addlinespace
Ratio of Immigration (90-00) x DumD05t09&            &            &            &    1.268   &    1.655   \\
               &            &            &            &  (0.965)   &  (1.050)   \\
\addlinespace
Ratio of Art, Enter, and Recre Emp (1999) x DumD99t05&            &            &            &            &    0.491   \\
               &            &            &            &            &  (0.525)   \\
\addlinespace
Ratio of Art, Enter, and Recre Emp (1999) x DumD05t09&            &            &            &            &   -2.276***\\
               &            &            &            &            &  (0.840)   \\
\addlinespace
Ratio of Health Emp (1999) x DumD99t05&            &            &            &            &   -0.434   \\
               &            &            &            &            &  (0.547)   \\
\addlinespace
Ratio of Health Emp (1999) x DumD05t09&            &            &            &            &    2.496** \\
               &            &            &            &            &  (1.184)   \\
\addlinespace
Ratio of Tradable Service Emp (1999) x DumD99t05&            &            &            &            &    0.127   \\
               &            &            &            &            &  (0.373)   \\
\addlinespace
Ratio of Tradable Service Emp (1999) x DumD05t09&            &            &            &            &    1.188   \\
               &            &            &            &            &  (0.756)   \\
\addlinespace
Ratio of College Students (1999) x DumD99t05&            &            &            &            &    0.165   \\
               &            &            &            &            &  (0.452)   \\
\addlinespace
Ratio of College Students (1999) x DumD05t09&            &            &            &            &   -0.290   \\
               &            &            &            &            &  (0.738)   \\
\midrule
Obs            &     1580   &     1580   &     1400   &     1400   &     1400   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   \\
KP F-Stat (99-05, non-stack sample)       &    10.99   &    13.02   &    7.889   &    10.46   &    9.267   \\
MOP F-Stat (99-05, non-stack sample)  &    9.896   &    12.26   &    7.322   &    10.04   &    8.726   \\
CoefEqual\_Chi2 &    8.974   &   10.377   &    5.999   &    7.162   &    6.538   \\
CoefEqual\_PValue &    0.003   &    0.001   &    0.014   &    0.007   &    0.011   \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}

==> Table_HH/table_RefineHouse.D00t06vsD07t10.HHDTI.2SLS.tex <==
%-----------------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_RefineHouse.D00t06vsD07t10.HHDTI.2SLS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Stacked Regression of Refined House Employment Growth in Boom (00-06) and Bust (07-10) Periods on Household Leverage Rise (99-05)} \smallskip \newline
{\scriptsize
This table reports 2SLS regression $\triangle_{00,06} \& \triangle_{07,10} RefinedHouseEmpShr_{c} = \beta_{00,06} * \triangle_{99,05} HHDTI_{c} \times Dum_{00,06} + \beta_{07,10} * \triangle_{99,05} HHDTI_{c} \times Dum_{07,10} + \gamma_{00,06}* \bm{Controls_{c}} \times Dum_{00,06} + \gamma_{07,10}* \bm{Controls_{c}} \times Dum_{07,10} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{00,06} \& \triangle_{07,10} RefinedHouseEmpShr_{c}$ is the change of the refined house employment share in working-age population at county $c$ 00-06 and 07-10. To reduce the impact of outliers, the dependent variable is winsorized at 5\% and 95\% levels in each period. The key independent variable $\triangle_{99,05} HHDTI_{c}$ is the rise in household leverage (debt-to-income ratio) at county $c$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in the period start year 1999. We use the gravity model-based instrumental variable $\triangle_{99,05}\text{givNetExp}_{m}$ as the IV for $\triangle_{99,05}HHDTI_{c}$. Regression is weighted by the natural logarithm of housing units in 1999.  For the first-stage F-test of two non-stacked samples, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
\smallskip
} % end of small font size
} % end of caption
\label{table_RefineHouse.D00t06vsD07t10.HHDTI.2SLS}

\vspace{-2mm}

\resizebox{0.55\columnwidth}{!}{%
\begin{tabular}{l*{4}{c}}
\toprule
\textbf{TSLS estimates}            &\multicolumn{4}{c}{Refined House Employment Growth x 100 (00-06 and 07-10, An)} \\
            \cmidrule{2-5} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
            
\midrule
HH Debt-to-Income Rise (99-05, An) x Dum00t06&    0.446** &    0.391** &    0.422*  &    0.421** \\
               &  (0.180)   &  (0.164)   &  (0.230)   &  (0.198)   \\
\addlinespace
HH Debt-to-Income Rise (99-05, An) x Dum07t10&   -0.785***&   -0.599***&   -0.680** &   -0.696** \\
               &  (0.254)   &  (0.221)   &  (0.336)   &  (0.318)   \\
\addlinespace
Dum00t06       &   -0.025   &    0.027   &   -0.162   &    0.012   \\
               &  (0.026)   &  (0.159)   &  (0.142)   &  (0.266)   \\
\addlinespace
Dum07t10       &    0.028   &    0.377   &    0.680***&   -0.104   \\
               &  (0.037)   &  (0.238)   &  (0.238)   &  (0.419)   \\
\addlinespace
Ln(Num of HH, 99) x DumD00t06&            &    0.015***&   -0.046   &   -0.033   \\
               &            &  (0.005)   &  (0.039)   &  (0.030)   \\
\addlinespace
Ln(Num of HH, 99) x DumD07t10&            &   -0.030***&    0.075   &    0.044   \\
               &            &  (0.008)   &  (0.056)   &  (0.048)   \\
\addlinespace
Ln(HH Income, 99) x DumD00t06&            &   -0.016   &   -0.002   &   -0.019   \\
               &            &  (0.021)   &  (0.019)   &  (0.030)   \\
\addlinespace
Ln(HH Income, 99) x DumD07t10&            &   -0.009   &   -0.026   &    0.046   \\
               &            &  (0.032)   &  (0.032)   &  (0.047)   \\
\addlinespace
Ratio of Labor Force (1999) x DumD00t06&            &   -0.060   &   -0.044   &   -0.073   \\
               &            &  (0.062)   &  (0.101)   &  (0.110)   \\
\addlinespace
Ratio of Labor Force (1999) x DumD07t10&            &    0.077   &    0.017   &    0.096   \\
               &            &  (0.101)   &  (0.162)   &  (0.186)   \\
\addlinespace
Ln(Num of HU, 99) x DumD00t06&            &            &    0.059   &    0.046   \\
               &            &            &  (0.043)   &  (0.033)   \\
\addlinespace
Ln(Num of HU, 99) x DumD07t10&            &            &   -0.106*  &   -0.076   \\
               &            &            &  (0.062)   &  (0.052)   \\
\addlinespace
Housing supply elasticity x DumD00t06&            &            &    0.004   &    0.003   \\
               &            &            &  (0.004)   &  (0.003)   \\
\addlinespace
Housing supply elasticity x DumD07t10&            &            &   -0.006   &   -0.006   \\
               &            &            &  (0.007)   &  (0.006)   \\
\addlinespace
House Vacancy Rate (1999) x DumD00t06&            &            &   -0.029   &   -0.022   \\
               &            &            &  (0.119)   &  (0.103)   \\
\addlinespace
House Vacancy Rate (1999) x DumD07t10&            &            &    0.049   &    0.053   \\
               &            &            &  (0.166)   &  (0.148)   \\
\addlinespace
Ratio of Renters (1999) x DumD00t06&            &            &    0.113   &    0.120   \\
               &            &            &  (0.093)   &  (0.111)   \\
\addlinespace
Ratio of Renters (1999) x DumD07t10&            &            &   -0.148   &   -0.115   \\
               &            &            &  (0.147)   &  (0.181)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x DumD00t06&            &            &            &    0.075   \\
               &            &            &            &  (0.072)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x DumD07t10&            &            &            &   -0.293** \\
               &            &            &            &  (0.126)   \\
\addlinespace
Ratio of White Race (1999) x DumD00t06&            &            &            &    0.008   \\
               &            &            &            &  (0.036)   \\
\addlinespace
Ratio of White Race (1999) x DumD07t10&            &            &            &    0.016   \\
               &            &            &            &  (0.044)   \\
\addlinespace
Ratio of Immigration (90-00) x DumD00t06&            &            &            &   -0.127   \\
               &            &            &            &  (0.302)   \\
\addlinespace
Ratio of Immigration (90-00) x DumD07t10&            &            &            &    0.322   \\
               &            &            &            &  (0.464)   \\
\midrule
Obs            &     1578   &     1578   &     1396   &     1396   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   \\
KP F-Stat (99-05, non-stack sample)       &    11.21   &    13.66   &    7.745   &    10.34   \\
MOP F-Stat (99-05, non-stack sample)  &    10.11   &    12.95   &    7.178   &    9.921   \\
CoefEqual\_Chi2  &    8.508   &    7.159   &    4.042   &    4.957   \\
CoefEqual\_PValue  &    0.004   &    0.007   &    0.044   &    0.026   \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}

==> Table_HH/table_Tradable.D00t06vsD07t10.NEP.D99t05.2SLS.tex <==
%-----------------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_Tradable.D00t06vsD07t10.NEP.D99t05.2SLS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Stacked Regression of Tradable Employment Growth in Boom (00-06) and Bust (07-10) Periods on Net Export Growth (99-05)} \smallskip \newline
{\scriptsize
This table reports 2SLS regression $\triangle_{00,06} \& \triangle_{07,10} TradableEmpShr_{c} = \beta_{00,06} * \triangle_{99,05} \text{NetExp}_{m} \times Dum_{00,06} + \beta_{07,10} * \triangle_{99,05} \text{NetExp}_{m} \times Dum_{07,10} + \gamma_{00,06}* \bm{Controls_{c}} \times Dum_{00,06} + \gamma_{07,10}* \bm{Controls_{c}} \times Dum_{07,10} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{00,06} \& \triangle_{07,10} TradableEmpShr_{c}$ is the change of the Tradable employment share in working-age population at county $c$ 00-06 and 07-10. The key independent variable $\triangle_{99,05} \text{NetExp}_{m}$ is the growth rate of net export growth in metropolitan area $m$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in the period start year 1999. We use the gravity model-based instrumental variable $\triangle_{99,05}\text{givNetExp}_{m}$ as the IV for $\triangle_{99,05}\text{NetExp}_{m}$. Regression is weighted by the natural logarithm of housing units in 1999.  For the first-stage F-test of two non-stacked samples, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
\smallskip
} % end of small font size
} % end of caption
\label{table_Tradable.D00t06vsD07t10.NEP.D99t05.2SLS}

\vspace{-2mm}

\resizebox{0.55\columnwidth}{!}{%
\begin{tabular}{l*{4}{c}}
\toprule
\textbf{TSLS estimates}            &\multicolumn{4}{c}{Tradable Employment Growth (00-06 and 07-10, An)} \\
            \cmidrule{2-6} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
            
\midrule
Net Export Growth (99-05, An) x Dum00t06&    0.790***&    0.804***&    0.701***&    0.742***\\
               &  (0.191)   &  (0.191)   &  (0.173)   &  (0.174)   \\
\addlinespace
Net Export Growth (99-05, An) x Dum07t10&    0.783***&    0.814***&    0.776***&    0.835***\\
               &  (0.215)   &  (0.228)   &  (0.249)   &  (0.259)   \\
\addlinespace
Dum00t06       &   -0.001***&    0.004   &    0.007   &    0.045***\\
               &  (0.000)   &  (0.006)   &  (0.007)   &  (0.016)   \\
\addlinespace
Dum07t10       &   -0.002***&    0.009   &    0.004   &    0.057***\\
               &  (0.000)   &  (0.007)   &  (0.009)   &  (0.019)   \\
\addlinespace
Ln(Num of HH, 99) x DumD00t06&            &   -0.000   &    0.006*  &    0.007*  \\
               &            &  (0.000)   &  (0.004)   &  (0.004)   \\
\addlinespace
Ln(Num of HH, 99) x DumD07t10&            &   -0.000   &    0.000   &    0.000   \\
               &            &  (0.000)   &  (0.002)   &  (0.002)   \\
\addlinespace
Ln(HH Income, 99) x DumD00t06&            &   -0.000   &   -0.001   &   -0.004***\\
               &            &  (0.001)   &  (0.001)   &  (0.002)   \\
\addlinespace
Ln(HH Income, 99) x DumD07t10&            &   -0.000   &   -0.000   &   -0.005***\\
               &            &  (0.001)   &  (0.001)   &  (0.002)   \\
\addlinespace
Ratio of Labor Force (1999) x DumD00t06&            &    0.000   &   -0.004   &   -0.005   \\
               &            &  (0.004)   &  (0.004)   &  (0.004)   \\
\addlinespace
Ratio of Labor Force (1999) x DumD07t10&            &   -0.009** &   -0.006   &   -0.006   \\
               &            &  (0.004)   &  (0.004)   &  (0.005)   \\
\addlinespace
Ln(Num of HU, 99) x DumD00t06&            &            &   -0.006*  &   -0.007*  \\
               &            &            &  (0.004)   &  (0.004)   \\
\addlinespace
Ln(Num of HU, 99) x DumD07t10&            &            &   -0.000   &   -0.001   \\
               &            &            &  (0.002)   &  (0.002)   \\
\addlinespace
Housing supply elasticity x DumD00t06&            &            &    0.000   &    0.000   \\
               &            &            &  (0.000)   &  (0.000)   \\
\addlinespace
Housing supply elasticity x DumD07t10&            &            &   -0.000   &   -0.000   \\
               &            &            &  (0.000)   &  (0.000)   \\
\addlinespace
House Vacancy Rate (1999) x DumD00t06&            &            &    0.012** &    0.011** \\
               &            &            &  (0.006)   &  (0.006)   \\
\addlinespace
House Vacancy Rate (1999) x DumD07t10&            &            &    0.009** &    0.007*  \\
               &            &            &  (0.004)   &  (0.004)   \\
\addlinespace
Ratio of Renters (1999) x DumD00t06&            &            &   -0.002   &   -0.006** \\
               &            &            &  (0.002)   &  (0.003)   \\
\addlinespace
Ratio of Renters (1999) x DumD07t10&            &            &    0.001   &   -0.006** \\
               &            &            &  (0.002)   &  (0.003)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x DumD00t06&            &            &            &    0.011** \\
               &            &            &            &  (0.005)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x DumD07t10&            &            &            &    0.014***\\
               &            &            &            &  (0.005)   \\
\addlinespace
Ratio of White Race (1999) x DumD00t06&            &            &            &    0.001   \\
               &            &            &            &  (0.001)   \\
\addlinespace
Ratio of White Race (1999) x DumD07t10&            &            &            &   -0.001   \\
               &            &            &            &  (0.002)   \\
\addlinespace
Ratio of Immigration (90-00) x DumD00t06&            &            &            &    0.012   \\
               &            &            &            &  (0.008)   \\
\addlinespace
Ratio of Immigration (90-00) x DumD07t10&            &            &            &    0.022** \\
               &            &            &            &  (0.009)   \\
\midrule
Obs            &     1578   &     1578   &     1396   &     1396   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   \\
KP F-Stat (99-05, non-stack sample)       &    23.44   &    23.20   &    16.52   &    17.83    \\
MOP F-Stat (99-05, non-stack sample)  &    22.98   &    22.71   &    16.16   &    17.49    \\
CoefEqual\_Chi2  &    0.001   &    0.002   &    0.117   &    0.183   \\
CoefEqual\_PValue  &    0.973   &    0.961   &    0.732   &    0.669   \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}
